New Nonexistence Results on Circulant Weighing Matrices

A circulant weighing matrix $W = (w_{i,j})$ is a square matrix of order $n$ and entries $w_{i,j}$ in $\{0, \pm 1\}$ such that $WW^T=kI_n$. In his thesis, Strassler gave a table of existence results for such matrices with $n \leq 200$ and $k \leq 100$. In the latest version of Strassler's table given by Tan \cite{arXiv:1610.01914} there are 34 open cases remaining. In this paper we give nonexistence proofs for 12 of these cases, report on preliminary searches outside Strassler's table, and characterize the known proper circulant weighing matrices.

==> Tex.tex <==
%%%%%%%%%% def's newcommand's, renewcommand's %%%%%%%%%%%%%%

\def\paira#1{{\langle{#1}\rangle}} % a pair of angles < >
\def\ddd#1{{\downarrow\!\!{#1}}}
\def\uuu#1{{\uparrow\!\!{#1}}}
\def\uudd#1{{\updownarrow\!\!{#1}}}
\def\from{\leftarrow}
\def\Size{\mathop{\rm Size}\nolimits}              % probability

\def\nauty/{{\tt nauty}}
\def\magma/{{\tt magma}}
\def\Magma/{{\tt Magma}}

\def\pderiv#1#2{{\partial{#1} \over \partial{#2}}} % partial deriv

% have equation labels include section number
%\def\theequation{\thesection.\arabic{equation}}

% for marginal comments %%%%%
\newcommand{\sside}[1]{% for silent side comments  w/o [???]
\marginpar{\tiny\raggedright #1}}
\newcommand{\side}[1]{ % for side comments w/ [???] in text
{\bf[???]}%
\sside{#1}}

%\newtheorem{question}{Question} % numbered vs unnumbered?  2004 aug 15
%\newtheorem{idea}{Idea} % numbered vs unnumbered?  2004 aug 15

%% \newtheorem{theorem}{Theorem}
%% \newtheorem{lemma}{Lemma}[section]
%% \newtheorem{conjecture}[theorem]{Conjecture}
%% \newtheorem{remark}{Remark}
%% \newtheorem{claim}{Claim}
%% \newtheorem{corollary}{Corollary}[section]
%% \newtheorem{proposition}{Proposition}[section]
%% \newtheorem{definition}{Definition}[section]

\def\myskip{{\vspace{0.3cm}}}

\def\eqref#1{(\ref{#1})}    			% for refs to equations

\def\al{\alpha}
\def\be{\beta}
\def\de{\delta}
%\def\ga{\gamma}
\def\ga{p}  % replace garble gamma by error probability p
\def\g{e}  % replace garble weight g by e
\newcommand{\ep}{\varepsilon}            % for ccr demands
\newcommand{\epsi}{\varepsilon}            % was rho in a previous version
\def\epsimax{{\epsi_{\max}}}
\def\De{\Delta}
\def\si{\sigma}
\def\ze{\zeta}

\def\cB{{\cal B}}
\def\cC{{\cal C}}
\def\cD{{\cal D}}
\def\cG{{\cal G}}
\def\cH{{\cal H}}
\def\cN{{\cal N}}
\def\cO{{\cal O}}
\def\cP{{\cal P}}
\def\cQ{{\cal Q}}
\def\cR{{\cal R}}
\def\cS{{\cal S}}
\def\cT{{\cal T}}
\def\cV{{\cal V}}

%\def\sA{{\sf A}}
%\def\sB{{\sf B}}
\def\sC{{\hbox{\sf\slshape C}}}
\def\sD{{\hbox{\sf\slshape D}}}
\def\sE{{\hbox{\sf\slshape E}}}
\def\sF{{\hbox{\sf\slshape F}}}
\def\sG{{\hbox{\sf\slshape G}}}
\def\sH{{\hbox{\sf\slshape H}}}
\def\sP{{\hbox{\sf\slshape P}}}
\def\sS{{\hbox{\sf\slshape S}}}
\def\sT{{\hbox{\sf\slshape T}}}
\def\sW{{\hbox{\sf\slshape W}}}
\def\sR{{\hbox{\sf\slshape R}}}

\def\bsP{{\underline{\sP}}}
\def\bsS{{\underline{\sS}}}

\def\cc{\mathbf{c}}
\def\ee{\mathbf{e}}
\def\gg{\mathbf{e}}
\def\vv{\mathbf{v}}
\def\ww{\mathbf{w}}
\def\xx{\mathbf{x}}
\def\yy{\mathbf{y}}

\newcommand{\cyc}[1]{\mathop{{\bf Q}(\zeta_{#1})}}
\newcommand{\zet}[1]{\mathop{\zeta_{#1}}}
\newcommand{\tw}[1]{\mathop{\theta_{#1}}}
\newcommand{\twx}[1]{\mathop{\theta_{#1}(x)}}
\newcommand{\zt}[1]{\mathop{\zeta_{#1}}}
\newcommand{\twb}[1]{\mathop{\theta_{[{#1}]}}}
\newcommand{\tz}[1]{\mathop{\theta(\zeta_{{#1}}})}
\newcommand{\tzbar}[1]{\mathop{\theta(\overline{\zeta_{{#1}}}})}
\newcommand{\twbx}[1]{\mathop{\theta_{[{#1}]}(x)}}

\newcommand{\br}[1]{\langle {#1} \rangle }

\newcommand{\bbr}[1]{\mathbf {\langle {#1} \rangle }}

\newcommand{\fa}{\mbox{$\mathfrak{a}$}}
\newcommand{\fb}{\mbox{$\mathfrak{b}$}}
\newcommand{\fp}{\mbox{$\mathfrak{p}$}}
\newcommand{\fq}{\mbox{$\mathfrak{q}$}}

\def\gv{{\hbox{\sf gv}}}
\def\hkl{{\hbox{\sf hkl}}}
\def\shannon{{\hbox{\sf s}}}
\def\shannonnk{{\shannon[n,k]}}
\def\shannonnde{{\shannon[n;\de]}}
\def\shannonde{{\shannon[\de]}}

%\def\vg{{\vec{g}}}                 % for garble vector

\def\Fnum{{\mathbb{F}}} % a field F
\def\Qnum{{\mathbb{Q}}} % a field F
\def\Nnum{{\mathbb{N}}} % a field F
\def\Cnum{{\mathbb{C}}} % a field F
\def\Znum{{\mathbb{Z}}} % a field F
\def\Rnum{{\mathbb{R}}} % a field R

\def\one{\mathbf{1}}
\def\zero{\mathbf{0}}
\def\val{\mathop{\rm val}\nolimits}              % probability
\def\len{\mathop{\rm len}\nolimits}              % probability
\def\prob{\mathop{\rm Prob}\nolimits}              % probability
\def\normm#1{{\|{#1}\|}}        % pair of lines with the norm
\def\floor#1{{\lfloor{#1}\rfloor}}
\def\sumno{\sum\nolimits}
\def\prodno{\prod\nolimits}

\def\rhomax{{\rho_{\max}}}

\def\endsurd{\hbox{ $\surd\!\!\!\!\surd$}}

% Fixing latex.tex's eqnarray:
%   simply adding a new dimension for this spacing.
\newdimen\eqnarraycolsep
\eqnarraycolsep .4\arraycolsep

\makeatletter
\def\eqnarray{\stepcounter{equation}\let\@currentlabel=\theequation
\global\@eqnswtrue
\global\@eqcnt\z@\tabskip\@centering\let\\=\@eqncr
$$\halign to \displaywidth\bgroup\@eqnsel\hskip\@centering
  $\displaystyle\tabskip\z@{##}$&\global\@eqcnt\@ne
  \hskip 2\eqnarraycolsep \hfil${##}$\hfil
  &\global\@eqcnt\tw@ \hskip 2\eqnarraycolsep
  $\displaystyle\tabskip\z@{##}$\hfil
   \tabskip\@centering&\llap{##}\tabskip\z@\cr}

% having references typed out

\def\thebibliography#1{\section*{References\@mkboth
 {REFERENCES}{REFERENCES}}\typeout{references:}
% \bibtoc	% added to have bibliography in table of contents
 \list
 {[\arabic{enumi}]}{\settowidth\labelwidth{[#1]}\leftmargin\labelwidth
 \advance\leftmargin\labelsep
 \usecounter{enumi}}
 \def\newblock{\hskip .11em plus .33em minus .07em}
 \sloppy\clubpenalty4000\widowpenalty4000
 \sfcode`\.=1000\relax}

\makeatother

\def\bibtoc{\addcontentsline{toc}{section}{References}}	% add bib to toc

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Taken from Arvind Borde, Mathematical TeX by Example, 1993
%   pages: 218, 222
%
% Peter Ostapenko 22-oct-93
% See /usr/local/papers/doc/doc-tex.tex for a version by Joe Weening
% Peter Ostapenko 6-may-94:
%   Control-A () for escape character
%   Control B () for whitespace
% Peter Ostapenko 9 oct 98
%   font size as in latex2e
% Peter Ostapenko 20 oct 98
%   fixing message comments
% Peter Ostapenko 28 oct 98
%   dealing with other control characters
% Peter Ostapenko 2004 apr 9
%   moving messages to when using command
%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

% IDEA:
% Minimal category codes needed to process TeX are:
%  1. escape (usually \)
%  2. whitespace ()
% We redefine category codes so that two ascii characters unused in
% the verbatim material are given these category codes.
%
% See p. 37, 367-370 of ``The TeXbook''

%\newcommand{\cc}{\catcode}

\def\beginliteral{%
\message{------------------------------------------------------------}%
\message{LITERAL.TEX: for TeXing visible ascii character material}%
\message{NB:}%
\message{..1. Control-A and Control-B should not appear in material.}%
\message{...... Used for escape and whitespace, respectively.}%
\message{..2. `endliteral' should not appear in material.}%
\message{..3. Should `untabify' material (e.g., using emacs command)}%
\message{...... to avoid misalignments from improper tab processing by TeX.}%
\message{..4. Should compare TeX output w/ actual ascii to double-check}%
\message{...... for bugs in this code.}%
\message{------------------------------------------------------------}%
\begingroup
  \catcode`\\=12
  \catcode`\{=12
  \catcode`\}=12
  \catcode`\$=12
  \catcode`\&=12
  \catcode`\#=12
  \catcode`\^=12
  \catcode`\_=12
  \catcode`\ =12
  \catcode`\~=12
  \catcode`\%=12
  \catcode`\*=12
  \catcode`\"=12
  \catcode`\@=12
  \catcode`\^^A=0                %  used for \ in literal material
  \catcode`\^^B=10               %  used for whitespace in literal material
  \catcode`\^^C=12
  \catcode`\^^D=12
  \catcode`\^^E=12
  \catcode`\^^F=12
  \catcode`\^^G=12
  \catcode`\^^H=12
  \catcode`\^^I=12
  \catcode`\^^J=12
  \catcode`\^^K=12
  \catcode`\^^L=12
  \catcode`\^^M=12
  \catcode`\^^N=12
  \catcode`\^^O=12
  \catcode`\^^P=12
  \catcode`\^^Q=12
  \catcode`\^^R=12
  \catcode`\^^S=12
  \catcode`\^^T=12
  \catcode`\^^U=12
  \catcode`\^^V=12
  \catcode`\^^W=12
  \catcode`\^^X=12
  \catcode`\^^Y=12
  \catcode`\^^Z=12
  \obeyspaces
  \losenolines
  \parskip0pt
  \parindent0pt
  \tt
  \thatisit
  }

{\obeyspaces\gdef {\hglue.5em\relax}}

%{\catcode`\`=\active \gdef`{\relax\lq}}

{\catcode`\^^M=\active %
\gdef\losenolines{\catcode`\^^M=\active \def^^M{\leavevmode\endgraf}}}

{\catcode`\=0 \catcode`\\=12 catcode`^^M=active %
 gdefthatisit^^M#1\endliteral{#1endgroup%
   noindentignorespaces}}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Example usage:
%   the file junk.tex is to be treated as flat ascii
%   input typeset in \tt 10pt
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%
%       \input literal
%       \begingroup
%       \fontsize{10}{10}
%       \tt
%       \beginliteral
%       inputjunk
%       \endliteral
%       \endgroup
%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

